Adaptive Accelerated Gradient Descent Methods for Convex Optimization

This work proposes A$^2$GD, a novel adaptive accelerated gradient descent method for convex and composite optimization. Smoothness and convexity constants are updated via Lyapunov analysis. Inspired by stability analysis in ODE solvers, the method triggers line search only when accumulated perturbations become positive, thereby reducing gradient evaluations while preserving strong convergence guarantees. By integrating adaptive step size and momentum acceleration, A$^2$GD outperforms existing first-order methods across a range of problem settings.

==> backupwords.tex <==
First-order methods, which utilize gradient information to optimize objective functions, are extensively employed in machine learning for model training due to their computational efficiency and scalability to large-scale, data-driven applications \cite{BottouCurtisNocedal2018}. Among these methods, one of the most fundamental algorithms is \textit{gradient descent} (GD): $x_{k+1}=x_k-\alpha_k\gf(x_k)$. Despite its effectiveness, GD exhibits two significant challenges:

\begin{itemize}[leftmargin=10pt, topsep=0pt, partopsep=0pt]
    \item \textbf{Step Size Selection:} The convergence rate of GD depends on the choice of step size $\alpha_k$. An excessively small step size leads to slow convergence, while an overly large step size may cause divergence. When $f$ is $L$-smooth, the step size is typically chosen as $1/L$. However, note that $L$ is the global Lipschitz constant of $f$. Ideally, the step size should be adapted to reflect local smoothness, leaving considerable room for improvement.
    \item \textbf{Convergence Speed:} Even with the optimal step size by solving (\ref{eq:exact}), GD can still be particularly slow when optimizing objective functions that are ill-conditioned or contain flat regions.
\end{itemize}

Below we list several strategies for addressing these challenges and enhancing convergence within the framework of first-order methods.

\paragraph{Backtracking line search}
In backtracking line search, we star with a relatively large estimate of step size, and then iteratively reduce it until a specific condition is met. A common condition is the Armijo–Goldstein condition (sufficient decrease condition). Nestorov (2012) \cite{Nesterov2012GradientMF} also proposed a stopping condition for composite convex functions. Though step size can be nearly optimal and convergence guarantee can be rigorous, this approach involves extra gradient evaluations at each iteration, and is computationally expensive compared to regular GD.

\paragraph{Adaptivity}
There are adaptive choices of step sizes that do not introduce extra expensive computation cost and speed up convergence. A popular one is the Barzilai-Borwein method \cite{10.1093/imanum/8.1.141}. However, this method is heuristic and lacks convergence guarantee. More recently, Malitsky and Mishchenko (2023) \cite{Malitsky2023AdaptivePG} proposed a novel adaptive step size selection strategy that allows for larger step sizes while maintaining convergence guarantees. Although this approach demonstrates improved efficiency, it is important to recognize that the absence of acceleration mechanisms may limit its performance, particularly when applied to ill-conditioned optimization problems.

\paragraph{Acceleration}
In accelerated methods, a momentum term is introduced, enabling the use of not only current gradient information but also the past updating direction. Nestorov's accelerated gradient (NAG) method \cite{nesterov1983method} was shown to achieve the accelerated rate of convergence $1-\sqrt{\kappa}$ under the fixed parameter choice in knowledge of $L$ and $\mu$. % Chen et al. \cite{chen2019orderoptimizationmethodsbased} proposed a Hessian-driven Nestorov accelerated method (HNAG), in which a Hessian damping term is introduced to neutralize oscillations in NAG. These methods, despite acceleration and robustness, involves step sizes that rely on $L$ and $\mu$. 
In practice, the crucial parameters $L$ and $\mu$ are unknown to users, bringing extra work of parameter fine-tuning.

\begin{center}
    \textsc{CONTRIBUTION}
\end{center}
In this work, we integrate the concepts of adaptivity and acceleration to develop an efficient first order optimization method. Our method introduces only minimal additional computational cost per iteration compared to regular gradient methods. In contrast, it automatically adapts the parameters \(L\) and \(\mu\), significantly reducing the number of gradient evaluations required to achieve convergence, while maintaining a strong theoretical guarantee.
Specifically, we make the following contributions:

\begin{itemize}[leftmargin=10pt, topsep=0pt, partopsep=0pt]
    \item We develop a framework based on Lyapunov analysis for accurately estimating optimization errors and consider the accumulation error.
    \item We propose an adaptive accelerated gradient descent (A$^2$GD) method and establish its accelerated linear convergence rate within the Lyapunov framework. We claim that our A$^2$GD method is superior to AGD (adaptive/accelerated gradient descent) methods by combining both adaptivity and acceleration.
    \item We extend the proposed algorithm from the smooth convex setting to the composite optimization case 
    \begin{equation}
    \min_{x\in\R^n} f(x):= h(x)+g(x),
\end{equation}
where function $h$ is $\mu$-convex ($\mu\geq 0$), $L$-smooth and coercive, and function $g$ is convex but non-smooth and prox-friendly.. % lower semi-continuous (lsc) .
\end{itemize}

\begin{algorithm}
    \caption{Adaptive Gradient Descent Method (Ad-GD)}\label{alg:adaptiveGD3}
\begin{algorithmic}[1]
\STATE \textbf{Parameters}: $x_0\in\mathbb{R}^n$, $L_0>0$, $\mu_0>0$.
%, $\gamma_u>1$, $\gamma_d\in(0,1)$, $r>1$
        \FOR{$k=0,1,2,\cdots$}
            \STATE $x_{k+1} \gets x_k -\frac{1}{L_k}\gf(x_k)$
            \STATE $b_k^{(1)} \gets \frac{1}{2L_k}\|\gf(x_{k+1})-\gf(x_k)\|^2-D_f(x_k,x_{k+1})$
            \STATE $b_k^{(2)} \gets -\frac{1}{2L_k}\|\gf(x_{k})\|^2$
            \STATE $p_k \gets (1 + \frac{\mu_k}{L_k})^{-1} \left(p_{k-1}+ b_k^{(1)}+b_k^{(2)}\right)$
            \IF{$p_k>0$}
                \STATE use the adaptive backtracking to update $L_k$ such that $b_k^{(1)}\leq 0$
%                            \STATE $p_k \gets (1 + \frac{\mu}{L_k})^{-1} \left(p_{k-1}+ b_k^{(1)}+b_k^{(2)}\right)$
            \ENDIF
%            \IF{$b_k^{(1)}>0$} % adjust for the next step
%                \STATE $L_k\gets \gamma_u L_k$
%            \ELSE
%                \STATE $L_k\gets \gamma_d L_k$
%            \ENDIF
\STATE $L_k\gets \frac{\|\gf(x_k)-\gf(x_{k+1})\|^2}{2D_f(x_k,x_{k+1})}$
            \STATE $\mu_k \gets \min\{\mu_k,L_k\}$
        \ENDFOR
    \end{algorithmic}
\end{algorithm}




==> numerics_backup.tex <==

\iffalse
\paragraph{2D Linear Laplacian problem}
We consider the linear finite element method for solving the Poisson equation in two dimensions:
$$ 
- \Delta u = b \quad \text{in } \Omega, \quad u = 0 \quad \text{on } \partial\Omega.
$$
The domain $\Omega$ is taken to be the unit disk, discretized using a quasi-uniform triangulation $\mathcal{T}_h$. Using the \texttt{$i$FEM} package~\cite{chen:2008ifem}, we assemble the corresponding stiffness matrix $A$, and define the objective function as the quadratic form
$\displaystyle 
f(x) = \frac{1}{2} (x - x^*)^\top A (x - x^*),$
where $x^* \in \mathbb{R}^n$ is a fixed (but arbitrary) target point. The initial guess $x_0$ is drawn componentwise from $\mathrm{Unif}(0, 1)$.

It is well known that the condition number of $A$ satisfies $\kappa(A) = O(h^{-2}) = O(n)$. The parameters $L$ and $\mu$ are estimated as the largest and smallest eigenvalues of $A$, respectively, though such estimates may be inaccurate for large-scale problems. We use quasi-uniform meshes on the unit disk rather than structured grids on a square, where eigenvalue bounds are more readily available in closed form.

% While AOR-HB achieves an optimal $O(\sqrt{\kappa})$ complexity, its performance is sensitive to the accuracy of the strong convexity estimate $\mu$, and degrades significantly when this estimate is inaccurate. %(see the last column of Table~\ref{tab:Laplacian}, where $\mu/10$ is used). 
% In contrast, A$^2$GD remains robust under such uncertainty and consistently outperforms the classical NAG method, matching or exceeding AOR-HB with optimally tuned parameters.
A$^2$GD outperforms other baseline methods. A$^2$GD involves roughly 0.1 extra gradient evaluation for line search per iteration, demonstrating effectiveness of our line search-reduced approach.
\fi

\iffalse
\vskip -10pt
\begin{table}[htbp]
    \centering
    \caption{Performance comparison on 2D linear Laplacian problem.}
    \label{tab:Laplacian}
    \vskip 3pt
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccc|cc|cc|cc|cc|cc}
        \toprule
        \multicolumn{3}{c|}{Problem Size} & \multicolumn{2}{c|}{A$^2$GD} & \multicolumn{2}{c|}{AdProxGD} & \multicolumn{2}{c|}{NAG} & \multicolumn{2}{c|}{AOR-HB($\mu$)} & \multicolumn{2}{c}{AOR-HB($\mu/10$)}\\
        \cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
        $h$ & $n$ & $\kappa$ & \#Grad & Time & \#Grad & Time & \#Grad & Time & \#Grad & Time & \#Grad & Time \\
        \midrule
        $1/20$ & 1262 & 7.85e+02 & 184 & 0.01 & 895 & 0.04 & 583 & 0.03 & 248 & 0.01 & 382 & 0.01 \\
        $1/40$ & 5167 & 3.15e+03 & 303 & 0.07 & 3191 & 0.70 & 1205 & 0.18 & 418 & 0.07 & 783 & 0.12 \\
        $1/80$ & 20908 & 1.30e+04 & 607 & 0.56 & 10729 & 9.54 & 1651 & 1.20 & 699 & 0.57 & 1581 & 1.42 \\
        $1/160$ & 84120 & 5.32e+04 & 987 & 5.97 & (>20000) & - & 2902 & 13.54 & 1187 & 5.62 & 2563 & 10.63 \\ % 116.41
        \bottomrule
    \end{tabular}
    }
\end{table}

% \LC{add one more row on the bottom to test a larger size.}
%Though the edge is shrinking, our convergence rate is better throughout the run, allowing for faster convergence of the Lyapunov function.

%\iffalse
%\begin{figure}
%    \centering
%    \begin{minipage}{0.425\linewidth}
%        \centering
%        \includegraphics[trim=50 200 50 200, clip,width=\linewidth]{./graph/illustration.pdf}
%        \caption{Illustration of Algorithm \ref{alg:adaptiveHNAG}.
%        The blue line captures the theoretical upper bound of the real Lyapunov function value (depicted in black). Their difference is the extra goodness the algorithm achieves, reflected in the red line.} 
%        \label{fig:illustration}
%    \end{minipage}
%    \hfill
%    \begin{minipage}{0.425\linewidth}
%        \centering
%        \includegraphics[trim=0 200 50 200, clip,width=\linewidth]{./graph/compare_AORHB.pdf}
%        \caption{Performance of Adaptive HNAG with AORHB methods with different choice of parameters $(L,\mu)$ on the 2D Laplace problem with grid size $h=1/160$. Given an estimate for $L$ and $\mu$, legend $(\gamma_1,\gamma_2)$ means the AORHB method with $L\gets \gamma_1 L$, $\mu \gets \gamma_2\mu$.} 
%        \label{fig:compare_AORHB}
%    \end{minipage}
%\end{figure}
%\fi

%\begin{figure}
%        \centering
%        \includegraphics[trim=0 200 50 200, clip,width=0.5\linewidth]{./graph/compare_AORHB.pdf}
%        \caption{Performance of Adaptive HNAG with AORHB methods with different choice of parameters $(L,\mu)$ on the 2D Laplace problem with grid size $h=1/160$. Given an estimate for $L$ and $\mu$, legend $(\gamma_1,\gamma_2)$ means the AORHB method with $L\gets \gamma_1 L$, $\mu \gets \gamma_2\mu$.} 
%        \label{fig:compare_AORHB}
%\end{figure}

\vspace{-10 pt}
\begin{minipage}[htdp]{0.45\textwidth}
    \centering
    \includegraphics[trim=90 250 100 250, clip, width=0.8\linewidth]{./graph/laplace2d_h160_nonad.pdf}
    \captionsetup{hypcap=false}
    \captionof{figure}{A2GD compared to non-adaptive methods.}      \label{fig:laplace2d_nonadaptive}
\end{minipage}%
\hfill
\begin{minipage}[htdp]{0.5\textwidth}
    \centering
    \includegraphics[trim=90 250 100 250, clip, width=0.75\linewidth]{./graph/laplace2d_h160.pdf}
    \captionsetup{hypcap=false}
    \captionof{figure}{A2GD compared to adaptive methods.
} 
    \label{fig:laplace2d_adaptive}
\end{minipage}
\fi


\iffalse
\begin{figure}[htbp]
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[trim=50 200 50 200, clip,width=\linewidth]{./graph/laplace2d_1382d.pdf}
        \caption{Function value gap. $h=0.05$.} 
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[trim=50 200 50 200, clip, width=\linewidth]{./graph/laplace2d_5409d.pdf}
        \caption{Function value gap. $h=0.025$.} 
    \end{minipage}
% \end{figure}

% \begin{figure}[htbp]
    \centering
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[trim=50 200 50 200, clip,width=\linewidth]{./graph/laplace2d_21395d.pdf}
        \caption{Function value gap. $h=0.0125$.} 
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\linewidth}
        \centering
        \includegraphics[trim=50 200 50 200, clip,width=\linewidth]{./graph/laplace2d_85095d.pdf}
        \caption{Function value gap. $h=0.00625$.} 
    \end{minipage}
\end{figure}

\fi

\iffalse
\ZX{We also monitor the increase of iterations as the problem becomes more ill-conditioned. In the loglog graph \ref{fig:cond_iter}, the slope of the curve \texttt{AdProxGD} is 2, indicating that it takes $O(1/\kappa)$ steps to converge, the same bound as standard gradient descent method. The slope of the curve NAG and AOR-HB are both 1, thus it takes $O(1/\sqrt{\kappa})$ steps for both methods to converge, a standard result for accelerating methods. The curve \texttt{A$^2$GD} is even flatter, indicating that our model has a better increase rate than $O(1/\sqrt{\kappa})$, achieving a super-accelerated performance. }
\fi
%\begin{figure}[htbp]
%    \centering
%    \includegraphics[trim=0 200 50 200, clip,width=0.5\linewidth]{graph/21395_dim.pdf}
%    \caption{relative error curves on 2D Laplace problem, $h=1/80$}
%    \label{fig:laplace2d_h1/80}
%\end{figure}

\vskip -12pt

\iffalse
\begin{table}[htbp]
    \centering
    \caption{Performance comparison on 2D linear Laplacian problem, $\mathrm{tol}=10^{-6}$}
    \label{tab:results}
    \begin{tabular}{cc|cc|cc|cc|cc}
        \toprule
        \multicolumn{2}{c|}{Problem Size} & \multicolumn{2}{c|}{A$^2$GD} & \multicolumn{2}{c|}{AdProxGD} & \multicolumn{2}{c|}{NAG} & \multicolumn{2}{c}{AOR-HB} \\
        \cmidrule(lr){1-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
        $n$ & $\kappa$ & \#Grad & Time & \#Grad & Time & \#Grad & Time & \#Grad & Time \\
        \midrule
        1382 & 1.85e+04 & 585 & 0.05 & 19350 & 1.08 & 1845 & 0.10 & 948 & 0.03 \\
        5409 & 6.96e+04 & 1058 & 0.39 & 47909 & 9.79 & 3494 & 0.53 & 1542 & 0.25 \\
        21395 & 2.85e+05 & 1170 & 2.50 & 72340 & 119.50 & 3681 & 3.07 & 2906 & 2.85 \\
        85095 & 1.25e+06 & 967 & 6.99 & 43916 & 172.19 & 4473 & 14.85 & 5757 & 20.03 \\
        \bottomrule
    \end{tabular}
\end{table}

\begin{table}[htbp]
    \centering
    \caption{Performance comparison on 2D linear Laplacian problem, $\mathrm{tol}=10^{-6}$}
    \label{tab:results}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccc|cc|cc|cc|cc}
        \toprule
        \multicolumn{3}{c|}{Problem Size} & \multicolumn{2}{c|}{A$^2$GD} & \multicolumn{2}{c|}{AdProxGD} & \multicolumn{2}{c|}{NAG} & \multicolumn{2}{c}{AOR-HB} \\
        \cmidrule(lr){1-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11}
        $h$ & $n$ & $\kappa$ & \#Grad & Time & \#Grad & Time & \#Grad & Time & \#Grad & Time \\
        \midrule
        $1/20$ & 1262 & 7.85e+02 & 162 & 0.0157 & 895 & 0.0531 & 583 & 0.0243 & 248 & 0.0097 \\
        $1/40$ & 5166 & 3.15e+03 & 293 & 0.0986 & 3191 & 0.8953 & 1205 & 0.2632 & 418 & 0.1140 \\
        $1/80$ & 20908 & 1.30e+04 & 476 & 0.6452 & 10729 & 15.7238 & 1651 & 1.8269 & 699 & 0.8076 \\
        $1/160$ & 84120 & 5.32e+04 & 791 & 5.0575 & (>20000) & 131.1896 & 2902 & 14.5124 & 1187 & 6.1099  \\
        % $1/320$ & 337476 & 2.00e+06 & 5108 & - & (>20000) & 674.6259 & 7477 & 221.6707 & 6370 & 193.0680 \\
        
        \bottomrule
    \end{tabular}
    }
\end{table}
\fi


\iffalse
\begin{figure}
    \centering
    \includegraphics[trim=50 300 50 200, clip,width=0.5\linewidth]{./graph/cond_iter.pdf}
    \caption{loglog graph of the number of iterations to the condition number of the linear problem.}
    \label{fig:cond_iter}
\end{figure}
\fi

\iffalse
\subsubsection{Quartic Anisotropic Bowl function}
The anisotropic bowl function is a convex quartic function that exhibits directional dependence due to varying scaling along different coordinate axes. For a given dimension \( n \), the function is defined as:
\[
f(x) = \sum_{i=1}^{n} i x_i^4
\]
where \( x = (x_1, x_2, \dots, x_n) \in \mathbb{R}^n \).
\fi


==> section_concluding_remark.tex <==
% !TEX root =  A2GDiclr_2026.tex

\section{Concluding Remarks}
Numerical results demonstrate that A$^2$GD consistently outperforms existing adaptive and accelerated gradient methods. A key advantage of A$^2$GD is its fully adaptive design, which requires no problem-specific parameter tuning, making it broadly applicable across convex optimization problems.

%\paragraph{Limitations and Extensions.}  
%Theoretical guarantees for A$^2$GD rely on convexity to ensure the positivity of the Bregman divergence, which plays a central role in error analysis. Extending this framework to nonconvex settings remains challenging. Nonetheless, we provide preliminary evidence of its applicability in a composite $\ell_{1\text{-}2}$ problem, where the nonconvex component admits a closed-form proximal operator.
%
%\paragraph{Line Search Overhead.}  
%While empirical results show that line search contributes minimal computational overhead—typically requiring only a few iterations—its worst-case complexity remains unbounded. A tighter theoretical characterization of the line search cost is an important direction for future work.


==> section_statements.tex <==
\section{LLM usage}
In preparing this manuscript, large language models (LLMs) were employed exclusively to assist with language-related tasks, such as improving readability, grammar, and style. The models were not used for research ideation, development of methods, data analysis, or interpretation of results. All scientific content, including problem formulation, theoretical analysis, and experimental validation, was conceived, executed, and verified entirely by the authors. The authors bear full responsibility for the accuracy and integrity of the manuscript.
% \section{Alternative proof}
% \input{appendix_D}
\section{Ethics statement}
This work is purely theoretical and algorithmic, focusing on convex optimization methods. It does not involve human subjects, sensitive data, or applications that raise ethical concerns related to privacy, security, fairness, or potential harm. All experiments are based on publicly available datasets or synthetic data generated by standard procedures. The authors believe that this work fully adheres to the ICLR Code of Ethics.
\section{Reproducibility statement}
We have taken several measures to ensure the reproducibility of our results. All theoretical assumptions are explicitly stated, and complete proofs are provided in the appendix. For the experimental evaluation, we describe the setup, parameter choices, and baselines in detail in the main text. The source code for our algorithms and experiments are available as supplementary materials. Together, these resources should allow others to reproduce and verify our theoretical and empirical findings.

